CuLDA_CGS: Solving Large-scale LDA Problems on GPUs

Latent Dirichlet Allocation(LDA) is a popular topic model. Given the fact that the input corpus of LDA algorithms consists of millions to billions of tokens, the LDA training process is very time-consuming, which may prevent the usage of LDA in many scenarios, e.g., online service. GPUs have benefited modern machine learning algorithms and big data analysis as they can provide high memory bandwidth and computation power. Therefore, many frameworks, e.g. Ten- sorFlow, Caffe, CNTK, support to use GPUs for accelerating the popular machine learning data-intensive algorithms. However, we observe that LDA solutions on GPUs are not satisfying. In this paper, we present CuLDA_CGS, a GPU-based efficient and scalable approach to accelerate large-scale LDA problems. CuLDA_CGS is designed to efficiently solve LDA problems at high throughput. To it, we first delicately design workload partition and synchronization mechanism to exploit the benefits of mul- tiple GPUs. Then, we offload the LDA sampling process to each individual GPU by optimizing from the sampling algorithm, par- allelization, and data compression perspectives. Evaluations show that compared with state-of-the-art LDA solutions, CuLDA_CGS outperforms them by a large margin (up to 7.3X) on a single GPU. CuLDA_CGS is able to achieve extra 3.0X speedup on 4 GPUs. The source code is publicly available on https://github.com/cuMF/ CuLDA_CGS.

==> 09_related.tex <==
\section{Related Work}\label{sec:related}


topic models.
~\cite{lda2003} original lda paper.

~\cite{sigir99plsi} plsi model.


Big data.

LDA models.
~\cite{scc17lda} a new model for online service.
~\cite{kdd12context}.
~\cite{kdd16streamlda} a new model.


LDA optimizations.


~\cite{yahoo12}. yahoolda.





~\cite{canny2013bidmach} bidmach.

~\cite{vldb16warp} warp LDA.

~\cite{asplos14diannao} diannao.

~\cite{kdd12context} new model.

~\cite{kdd13cgs} improve the lda convergence speed.

~\cite{kdd16node} algorithm, other topics.

~\cite{kdd13graph} large-scale graph.

~\cite{kdd17topic} new model to reduce computing complexity.

TPU~\cite{isca17tpu}.

~\cite{kdd14alias} alisa LDA, reduce sampling complexity.

~\cite{asplos17saber} saber lda.

~\cite{kdd14batch} mini batch.

~\cite{kdd16cloud} large-scale SCD.

~\cite{kdd15bayeslda} minimize the memory consumption of LDA.

~\cite{kdd16topicmodel} novel algorithm.

~\cite{ppopp15gun} gpu-based graph processing lib.

~\cite{acm09roofline} roofline model.

~\cite{hpdc17mf} mf.

~\cite{kdd15pet}. distributed big data library.

~\cite{kdd16dislda} distributed LDA.

~\cite{kdd09sparse} sparsity-aware sampling.

~\cite{www15nomad}. discussed the f+tree.

~\cite{www15light} lightlda.

~\cite{vldb17yu} ldastar.

~\cite{kdd16shorttext} new model.





GPU in big data \& machine learning. . DianNao~\cite{asplos14diannao}.



